Towards a Neural Era in Dialogue Management for Collaboration: A Literature Survey

Dialogue-based human-AI collaboration can revolutionize collaborative problem-solving, creative exploration, and social support. To realize this goal, the development of automated agents proficient in skills such as negotiating, following instructions, establishing common ground, and progressing shared tasks is essential. This survey begins by reviewing the evolution of dialogue management paradigms in collaborative dialogue systems, from traditional handcrafted and information-state based methods to AI planning-inspired approaches. It then shifts focus to contemporary data-driven dialogue management techniques, which seek to transfer deep learning successes from form-filling and open-domain settings to collaborative contexts. The paper proceeds to analyze a selected set of recent works that apply neural approaches to collaborative dialogue management, spotlighting prevailing trends in the field. This survey hopes to provide foundational background for future advancements in collaborative dialogue management, particularly as the dialogue systems community continues to embrace the potential of large language models.

==> sections/rq1/frame-based.tex <==
\subsection{Limitations of Slot-Filling Approaches} \label{sec:frame}
In this section, we address the limitations of the prevalent slot-filling approach, which inadequately captures the nuances of collaborative dialogues. Despite success in customer service, information retrieval, and personal assistant domains, this approach lacks the expressivity for rich collaborative dialogue states \cite{cohen_back_2018, cohen_foundations_2019}. While acknowledging its prominence in dialogue systems research, we exclude it from our review due to its limitations.

Slot-filling or frame-based dialogue management employs structured representations known as frames \cite{bobrow1977gus, fillmore1977case} and has gained attention through virtual assistants like Siri, Alexa, and Google Assistant. However, it falls short in representing complex collaborative dialogue states \cite{cohen_back_2018, cohen_foundations_2019}. As a result, we focus on its limitations rather than its application in collaborative dialogues.

\citet{cohen_foundations_2019} provides a detailed critique of using intent + slot (I+S) combinations to represent utterance meanings. We highlight key limitations from this analysis in the context of an I+S representation.
\begin{enumerate}
    \item \textbf{Agent of the action unspecified.} In collaborative dialogue, it is common to delegate tasks and share the workload between agents. However, an I+S representation such as  \texttt{reserve(restaurant=Mykonos, cuisine=Greek, location=North} does not clarify \textit{who} needs to perform the action of reserving the table (is it the user or the system?).
    \item \textbf{Restriction on logical forms.} While not specific to collaborative contexts, this is another key limitation pertaining to the NLU side of things. Single atomic slot value for a \textit{time} slot (e.g., \textit{7 pm}, \textit{tomorrow}, etc.) cannot represent complex constructs such as \textit{not before 7 pm} or \textit{between 7 and 8 pm}.
    \item \textbf{Handling initiative shifts.} Consider the following three-turn exchange. U: \textit{what’s the earliest time available?}; S: \textit{6 pm}; U: \textit{too early}; S: \textit{How about 7 pm?}. Here, the user utterance \textit{too early} is an indirect request for the system to take the initiative in suggesting the value. However, this nuance would be lost in a I+S representation.
    \item \textbf{"Know if".} While I+S representation can capture both a request to John for Mary's phone number (\texttt{request\_phone(name=Mary)}) and his response (\texttt{inform(phone=123456789)}), it cannot represent facts such as \textit{John knows (or does not know) Mary's phone number}, which is different from both requesting for and informing the actual phone number. The capability to \textit{know if} another agent knows a fact is useful in collaborative situations to know, for example, to whom a question needs to be directed to.
\end{enumerate}

==> sections/rq2/disentangling.tex <==
\subsection{Decoupling Semantics and Surface Realizations}



\label{sec:disentangling}
In this section, I review approaches that address an important limitations of vanilla end-to-end trained models of dialogue: separation of semantics and surface realization. In vanilla sequence-to-sequence modeling of dialogue, a trained neural network processes raw dialogue history as input and directly generates the subsequent natural language response without distinct intermediate steps for natural language understanding, state tracking, and generation. Crucially, traditional end-to-end training approaches fail to distinguish between "what to say" (semantics) and "how to say it" (surface realization), leading to complications as a single concept can be expressed in numerous ways.

% From our analyzed works, we find 

%The term "end-to-end" describes the models' end-to-end differentiable characteristic. While end-to-end neural dialogue models offer benefits over pipeline-based architectures (elaborated in Section \ref{sec:rq1-e2e}), they encounter difficulties in strategic and collaborative contexts.

% Here, I review approaches used in my chosen set of works to decouple the semantics of response generation models from their corresponding surface-level natural language realizations.

% Some other issues with vanilla SL approaches include 1) reduced interpretability (crucial for trust in many collaborative applications) due to the absence of explicit underlying structure, 2) hallucinations \cite{ji2023survey} due to a lack of grounding (which can lead to contextually inappropriate or inconsistent responses), 3) generating uninteresting responses lacking in diversity \cite{lewis_deal_2017}, 3) requiring extensive training data, which may be scarce for specialized domains \cite{mehri2019structured}, 3) difficulty incorporating external knowledge \cite{madotto-etal-2018-mem2seq}. Researchers address these challenges by exploring disentangled representations and modifying neural sequence-to-sequence models.

\subsubsection{Conditioning Response Generation on Intermediate Symbolic Representations}
\citet{he-etal-2018-decoupling} propose an approach that separates a dialogue system's strategy from the natural language surface realization in a negotiation setting. They employ \textit{two} distinct sequence-to-sequence models to represent the dialogue (see Figure \ref{fig:he-negotiation}). The first model operates directly on the tokens in natural language utterances, while the second model works with coarse dialogue acts corresponding to the utterances. First, a parser is trained to map an utterance, $x_{t-1}$, to a coarse dialogue act $z_{t-1}$, which captures the high-level dialogue flow. A dialogue act consists of an intent and optional arguments. For instance, the utterance "I would like to pay \$125 for it. How does that sound?" is mapped to the dialogue act \texttt{propose(price=125)}. The dialogue act ontology includes \texttt{inform}, \texttt{inquire}, \texttt{propose}, \texttt{counter}, and \texttt{agree}. Both sequences are modeled using LSTMs \cite{hochreiter1997long}. Given $z_{t-1}$ and the dialogue history, $x_{<t}$, the dialogue manager predicts the coarse dialogue act of its response, $z_{t}$. Finally, a natural language response is generated based on $z_t$.

\archdiagram{rq2}{he-negotiation}{In \citet{he-etal-2018-decoupling}, the natural language parser generates dialogue acts, $z_{<t}$, corresponding to the utterances $x_{<t}$ respectively. The next response is generated in two steps: (1) generating the next dialogue act, $z_t$ based on the previous dialogue acts, $z_{<t}$ and 2) generating the natural language response based on both the dialogue history, $x_{<t}$ and the preceding dialogue act, $z_t$.}

% 
\citet{santhanam_learning_2020} present an approach that generates an intermediate "plan" to condition the natural language response. They demonstrate this method on the \textsc{Persuasion For Good} dialogue corpus \cite{wang2019persuasion}, in which the agent persuades a listener by offering compelling incentives. The process consists of two steps: first, generating a pseudo-natural language plan, and second, conditioning the model on this plan to produce the final response. Figure \ref{fig:santhanam} illustrates an example dialogue context along with a system-generated intermediate plan. In response to B's final utterance, the model first generates a plan with an \textit{ask} and \textit{framing}, such as \texttt{PERFORM [provides [relief]]}. It then creates a natural language response, such as \textit{"Save the Children is an international non-governmental organization that promotes children's rights, provides relief, and supports children in developing countries"} (surface realization).

\archdiagramhalf[0.5]{rq2}{santhanam}{Separation of NLG into planning and surface realization \cite{santhanam_learning_2020}.}


\subsubsection{Conditioning Response Generation on Latent Representations}
In contrast to approaches that employ symbolic intermediate representations like dialogue acts and plans, some methods utilize latent variables instead.

\citet{Yarats2017HierarchicalTG} propose generating a short-term plan using latent sentence representations. The natural language response is then generated by conditioning the response generation step on this plan. To learn these latent sentence representations from data, the authors deviate from the traditional paradigm of maximizing the likelihood of the current utterance $x_t$ given the latent representation $z_t$. Rather, they train $z_t$ to maximize the likelihood of the response at the \textit{next turn}, $x_{t+1}$. This approach is motivated by the observation that while the traditional method effectively models semantic similarity, it fails to capture the influence of an utterance on the dialogue partner's response. This distinction can be crucial in negotiation settings, where even subtle lexical substitutions such as using "two" instead of "one," can significantly affect the final outcomes of the conversation.

%When using supervised learning (SL) for end-to-end response generation, the model is penalized for not producing the exact response as the ground truth sample in the training dataset. This is unreasonable, as multiple ways to convey the same semantic meaning may exist. Furthermore, in strategic scenarios such as negotiation or planning, penalizing a model for not adhering to a single ground-truth utterance hinders exploration of alternative strategies to achieve the same goal. Empirical evidence reveals that basic SL results in significantly underperforming strategic dialogue agents compared to advanced approaches like reinforcement learning (RL) and the induction of disentangled representations \cite{cuayahuitl2015strategic}.



==> sections/rq2/rl.tex <==
\subsection{Training with Reinforcement Learning} \label{sec:rl}

Supervised learning 

